Adaptive Importance Sampling based Neural Network framework for Reliability and Sensitivity Prediction for Variable Stiffness Composite Laminates with hybrid uncertainties

In this work, we propose to leverage the advantages of both the Artificial Neural Network (ANN) based Second Order Reliability Method (SORM) and Importance sampling to yield an Adaptive Importance Sampling based ANN, with specific application towards failure probability and sensitivity estimates of Variable Stiffness Composite Laminate (VSCL) plates, in the presence of multiple independent geometric and material uncertainties. The performance function for the case studies is defined based on the fundamental frequency of the VSCL plate. The accuracy in both the reliability estimates and sensitivity studies using the proposed method were found to be in close agreement with that obtained using the ANN based brute-force MCS method, with a significant computational savings of 95\%. Moreover, the importance of taking into account the randomness in ply thickness for failure probability estimates is also highlighted quantitatively under the sensitivity studies section.

==> Mischellaneous.tex <==
\section{Structure}
\label{sec:1}
A paper for publication can be subdivided into multiple sections: a title, full names of all the authors and their affiliations, a concise abstract, a list of keywords, main text (including figures, equations, and tables), acknowledgements, references, and appendix. Running title is optional.

\subsection{Text Layout}
Acceptable paper size is US Letter (8.5''x11'' or 21.59 cmx27.94 cm). All margins-top, bottom, left, and right-are set to 1.5'' (3.81 cm). The paper must be single column, single spaced, except for the headings as outlined below. Acceptable font is Times New Roman, 11 pt., except for writing special symbols and mathematical equations.

\subsection{Headings}
Level one headings for sections should be in bold, and be flushed to the left. Level one heading should be numbered using Arabic numbers, such as 1, 2,...
Level two headings for subsections should be in bold-italic, and be flushed to the left. Level two headings should be numbered after the level one heading. For example, the second level two heading under the third level one heading should be numbered as 3.2.
Level three headings should be in italic, and be flushed to the left. Similarly, the level three headings should be numbered after the level two headings, such as 3.2.1, 3.2.2, etc.

\section{Equations and Mathematical Expressions}
Equations and mathematical expressions must be inserted into the main text. Two different types of styles can be used for equations and mathematical expressions. They are: In-line style and display style.

\subsection{In-line Style}
In-line equations/expressions are embedded into the paragraphs of the text. For example, $E = m{c^2}$. In-line equations or expressions should not be numbered and should use  the same/similar font and size as the main text.

\subsection{Display Style}
Equations in display format are separated from the paragraphs of the text. Equations should be flushed to the left of the column. Equations should be made editable. Displayed equations should be numbered consecutively, using Arabic numbers in parentheses. See Eq. (\ref{equ:1}) for an example. The number should be aligned to the right margin.
\begin{equation}
\label{equ:1}
E = m{c^2}
\end{equation}

\section{Figures and tables}
Figures and tables should be inserted in the text of the manuscript.

\subsection{Figures}
Figures should have relevant legends but should not contain the same information which is already described in the main text. Figures (diagrams and photographs) should also be numbered consecutively using Arabic numbers. They should be placed in the text soon after the point where they are referenced. Figures must be submitted in digital format, with resolution higher than 300 dpi.

\subsubsection{Figure format}
Figures should be centered, and should have a figure caption placed underneath. Captions should be centered in the column, in the format ``Figure 1. The text caption XXXX'', where the number of the figure follows the key word Figure, and the text caption comes right after that.
The size of the figure is measured in centimeters and inches. Please prepare your figures at the size within 17 cm (6.70 in) in width and 20 cm (7.87 in) in height. Figures should be in the original version , with no \textbf{stretchor} distortion.

\subsubsection{Figure labels and captions}
Figure labels must be sized in proportion to the image, sharp, and legible. Label size should be no smaller than 8-point and no larger than the font size of the main text. Labels must be saved using standard fonts (Arial, Helvetica or Symbol font) and should be consistent for all the figures. All labels should be in black, and should not be overlapped, faded, broken or distorted. A space must be inserted before measurement units. The first letter of each phrase, NOT each word, must be capitalized.
One-line Caption should be centered in the column, in the format of ''\textbf{Figure 1}. The text caption...'' That is, the number of the figure follows the keyword \textbf{Figure}, and next to it, the text caption. For one example, see Fig. (\ref{fig:1}) below.
\begin{figure*}[h]
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
\begin{center}
  \includegraphics[width=0.6\textwidth]{figure1.pdf}
\end{center}
% figure caption is below the figure
\caption{Macroscopic structure and microscopic unit cell }
\label{fig:1}       % Give a unique label
\end{figure*}

\subsection{Tables}
Tables should also be numbered consecutively using Arabic numbers. They should be placed in the text soon after the point where they are referenced. Tables should be centered and should have a table caption placed above. Captions should be centered in the format ''{\bf Table 1}. The text caption...''. For one example, see Tab. \ref{tab:1}.
\begin{table}
\caption{Table caption, such as 'Comparison of computing results for temperature increment in $L^2$-norm'}
\label{tab:1}       % Give a unique label
\centering
\begin{tabular}{cccc}
\hline\noalign{\smallskip}
 & $\frac{\|e_\theta^0\|_{L^\infty(L^2)}}{\|\theta_{FE}^\varepsilon\|_{L^\infty(L^2)}}$ & $\frac{\|e_\theta^1\|_{L^\infty(L^2)}}{\|\theta_{FE}^\varepsilon\|_{L^\infty(L^2)}}$  & $\frac{\|e_\theta^2\|_{L^\infty(L^2)}}{\|\theta_{FE}^\varepsilon\|_{L^\infty(L^2)}}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
Case 1 & 0.726833 & 0.727374 & 0.009774 \\
Case 2 & 0.720257	&0.720645	&0.014425 \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}

\section{Citations}
The author-year format of the citation must be used for the references. The author-year format of the citation must be used for the references. For example, [\cite{atluri2002meshless}]. If the cited reference has more than three authors, please see the example, [\cite{atluri2002meshless,atluri2003meshless,atluri1998new}]. If the cited reference has more than three authors, please cite all first three authors' last names, and followed by "et al.". For example, [\cite{atluri2003meshless}], [\cite{Duan2013a}]. When you cite more than one reference, please cite the name of the first author and year of each reference and separate them by a semicolon. If the sentence starts with a referenced author's name, please cite right after the author's name. For example, "Atluri \text {et al.} [\cite{atluri2004meshless}] have found that...". No citation to the page number should be used.

\section{References}
All references should be listed at the end of the paper. The names of the authors should be in bold, with the last name(s) first. The year in which the paper is published follows the name (s) of the author(s). Journal and book titles should be in italic. A full name of journal cited in reference should be used followed by a comma before the volume, issue and page number. Please see the examples below:
\acknowledge{The authors wish to express their appreciation to the reviewers for their helpful suggestions which greatly improved the presentation of this paper.}

% Numerical examples 
The Design of Experiment (DoE) was conducted as follows: in the first case, the geometrical parameters were kept deterministic and the material parameters were assumed to be random. In the second case, the reverse case was considered where the geometrical features were assumed to be random, keeping the material parameters at its deterministic setting. In both the cases, the probability of failure along with sensitivity studies are performed as a function of the CoV (Coefficient of Variation) of the input random material parameter. The effect of aspect ratio on the output response is also studied by considering two different values: $a/b = $ 1 and $a/b =$ 1/2.

In both cases, a sample set of $N_{\text{samples}}=$ 1000 was randomly chosen from the input parametric space and the first mode of vibration was numerically determined for each sample from the above set. Thereafter, the limit-state function value is evaluated for each of the recorded first mode of random frequency using the relation given in Equation \ref{eq:12}.

\textcolor{red}{\begin{itemize}
    \item Add a correlation plot showing the correlation between the predicted limite state function and original lsf using the training dataset. 
    \item Sensitivity study of prediction of reliability index proposed ANN method against the number of nodes in the hidden layer and and size of training dataset. 
    \item Consider symmetric and non-symmetric laminates. 
    \item Add results for the processing time Tp using finite element based MCS (how many samples ?) and neural networks. Tp values are presented as a percentage of the largest processing time for all simulations. Meanwhile, the computed processing time using ANN to evaluate Pf includes the training time, which is performed using finite elements.
\end{itemize}}

\begin{table}[htpb!]
\caption{Comparative values for relative processing time for several methods using neural networks and FEM based MCS for reliability analysis of a variable stiffness composite laminate plates with cutouts.}
\label{tab:7}       
\centering
%\resizebox{\textwidth}{!}
{\begin{tabular}{l l l l l l l} 
\hline\noalign{\smallskip}
Method & Relative processing time & Number of simulations (NS) & Number of failure points (NF) & Failure probability (Pf) & Coefficient of variation (Pf) & Reliability index ($\beta$) \\
\noalign{\smallskip}\hline\noalign{\smallskip}
Standard Monte Carlo (SMC) & & & & & & \\
Importance sampling (MC-IS) & & & & & & \\ 
FORM & & & & & & \\ 
ANN training & & & & & & \\  
SMC + trained ANN & & & & & & \\ 
MC-IS + trained ANN & & & & & & \\  
FORM + trained ANN & & & & & & \\  
\hline\noalign{\smallskip}
\end{tabular}}
\end{table}

% The constitutive equation for the $k^{\rm th}$ layer, in the orthotropic local coordinate derived from Hooke's law for the plane stress is given by:
% \begin{equation}
% \begin{Bmatrix}
% \sigma_1 \\ \sigma_2  \\ \sigma_{12} \\ \sigma_{13} \\ \sigma_{23}  \end{Bmatrix}^k = 
% \begin{bmatrix}
% Q_{11} & Q_{12} & Q_{13} & 0 & 0 \\ 
% Q_{21} & Q_{22} & Q_{23} & 0 & 0 \\ 
% Q_{31} & Q_{32} & Q_{33} & 0 & 0 \\ 
%   0    &  0     &   0    & Q_{44} & 0 \\ 
%   0    &  0     &   0    &   0    & Q_{55} 
% \end{bmatrix}^{k}   
% \begin{Bmatrix}
% \epsilon_1 \\ \epsilon_2 \\ \epsilon_{12} \\ 
% \epsilon_{13} \\ \epsilon_{12} 
% \end{Bmatrix}^{k}
% \label{eqn:sparseKuf}
% \end{equation}

% \noindent The engineering constants $Q_{ij}$ as functions of the longitudinal and the transverse modulus of elasticity $(E_1,E_2)$, Poisson's ratios $(\nu_{12},\nu_{21})$ and shear modulus $(G_{12},G_{13},G_{23})$ are given by:
% \begin{align}
%     Q_{11} &= E_1 / (1-\nu_{12} \nu_{21})  \nonumber \\ 
%     Q_{22} &= E_2 / (1-\nu_{12} \nu_{21})  \nonumber \\
%     Q_{12} &= \nu_{12}E_{12} / (1- \nu_{12}\nu_{21})  \label{eq:26}
% \end{align}
% and $Q_{12} = Q_{21}, Q_{33} = G_{12}, Q_{44} = G_{13}, Q_{55} = G_{23}$. Equation \ref{eq:4} - \ref{eq:26} represents the directions parallel and perpendicular to the fibre direction. By performing a proper coordinate transformation, the stress-strain relationships of a single $k^{\rm th}$ lamina in the $xyz$ coordinate can be obtained as:
% \begin{equation}
%     \begin{Bmatrix}
%         \sigma_{x} \\ \sigma_{y} \\ \sigma_{xy} \\
%         \sigma_{xz} \\ \sigma_{yz} 
%     \end{Bmatrix}^k
%     = 
%     \begin{bmatrix}
%         \overline{Q_{11}} & \overline{Q_{12}} & \overline{Q_{13}} & 0 & 0 \\
%         \overline{Q_{21}} & \overline{Q_{22}} & 
%         \overline{Q_{23}} & 0 & 0 \\
%         \overline{Q_{31}} & \overline{Q_{32}} & \overline{Q_{33}} & 0 & 0 \\
%         0 & 0 & 0 & \overline{Q_{44}} & \overline{Q_{45}} \\ 
%         0 & 0 & 0 & \overline{Q_{54}} & \overline{Q_{55}}
%     \end{bmatrix}^{k}
%     \begin{Bmatrix}
%         \epsilon_x \\ \epsilon_y \\ \epsilon_{xy} \\ \epsilon_{xz} \\ \epsilon_{yz}
%     \end{Bmatrix}^{k}
% \end{equation}

\begin{align} 
    E_d &= \frac{1}{2} \int_{xy} \left[ \sigma_{xx} \epsilon_{xx} + \sigma_{yy} \epsilon_{yy} + \tau_{xy} \gamma_{xy} + \tau_{xz} \gamma_{xz} + \tau_{yz} \gamma_{yz} \right] dxdy  \label{eq:520} \\ 
    E_c &= \frac{1}{2} \rho \int_{xy} \left[ \left( \frac{\partial u}{\partial t} \right)^2 + \left( \frac{\partial v}{\partial t} \right)^2 + \left( \frac{\partial w}{\partial t} \right)^2  \right] dxdy  \label{eq:521}
\end{align}


The Largrange equation of free motion is then given by: 

\begin{equation}
    \frac{d}{dt} \left(\frac{\partial E_c}{\partial q} \right) - \frac{\partial E_c}{\partial q} + \frac{\partial E_d}{\partial q} = 0 
\end{equation}

\noindent where $q$ are the degree of freedom in the system. By inserting the strain energy and the kinetic energy in the Lagrangian formulation, the equation of free motion can then be expressed as: 

\begin{equation}
    [M]\{\ddot{q}\} + [K] \{q\} = 0  
\end{equation}
where $[K]$ and $[M]$ are the stiffness and mass matrix respectively. 

% \begin{table}
% \caption{Types of activation function and their respective equations}
% \label{tab:1}       
% \centering
% \begin{tabular}{lccl}
% \hline\noalign{\smallskip}
%   & Activation function ($f(z)$) & Range & Remark \\
% \noalign{\smallskip}\hline\noalign{\smallskip}
% Identity &  $z$ & $<-\infty,\infty>$ & Not suitable for data \\
%  &  &  &with non-linear trend \\
% Heaviside (Binary step) &  $\begin{cases}
%     1,& \text{for } z\geq 0\\
%     0,& \text{for } z<0
% \end{cases}$ & [0,1] & Derivative at zero undefined\\
% Logistic (sigmoid) & $\dfrac{e^{z}}{1+e^z}$ &  $<0,1>$ & Mainly used in output layer \\
% Hyperbolic tangent & $\dfrac{e^z - e^{-z}}{e^z + e^{-z}}$ & $<-1,1>$ & Faster learning due to \\
% &  &  & higher derivatives\\ \\
% ReLU & ${\rm max}(0,z)$ & [0,$\infty>$ & Faster learning rate\\  \\
% Softplus & $\ln{(1+e^z)}$ & [0,$\infty>$ & Derivative at z=0 defined\\ 
% SoftMax &  $\dfrac{e^{z_i}}{\sum_{n=1}^{N}e^{z_n}}$ & $<0,1>$ & Relies on entire net input\\
% \noalign{\smallskip}\hline
% \end{tabular}
% \end{table}

% \begin{figure}[htbp!]  
% \centering
% \includegraphics[width=1\textwidth]{./Figures/Activation_function.eps}
% \caption{Commonly used activation function in neural network literature: logistic, sigmoid, hyperbolic, tangent(tanh),softplus and ReLU.}
% \label{fig:Activation_function}
% \end{figure} 

%In the present study, the set of random variables constitute the following: 
% \begin{equation}
% \begin{split}
%     \mathbf{X} &= [E_{11},E_{22},G_{12},d,c/d,x_c,y_c,\theta_{0,1},\theta_{0,2},\cdots, \theta_{0,N_L}\\ & \qquad t_1,t_2,\cdots,t_{N_L}]
% \end{split}
% \end{equation}
%\noindent The first three parameters captures the randomness in material parameters. $\theta_{0,k}$ represents the fibre angle values at $x = 0$ for each ply. Similarly, $t_i : i=1,2,\cdots,N_L$ stands for the random ply thickness values. Finally, the random parameters $d$ and $c/d$ represents the major axis and ellipticity of cutout, while $x_c$ and $y_c$ is the random location of its center.

Based on the adopted definition of the performance function as in Eq. \ref{eq:12}, a failure surface or a limit state of interest can be defined as $g(\mathbf{X})=0$, with the failure probability being defined as follows: 

\begin{equation} \label{eq:14}
    P_f = \int \cdots \int_{g(\mathbf{X})<0} f_X (x_1,x_2,\cdots,x_N) dx_1 dx_2 \cdots dx_N
\end{equation}

\noindent where $f_X(x_1,x_2,\cdots,x_N)$ is the joint PDF of the $N$ random variables. It should be observed that the above integration is performed only over the failure region $g(\mathbf{X})<0$. %In this section, the mathermatics behind two of the most commonly used Reliability Methods namely FORM and SORM will be outlined for the interest of the reader, along with the computation of the Most Probable failure Point (MPP). 

Failure probability is defined as the probability of a performance function g($\mathbf{X}$) is less than zero, where $\mathbf{X}$ is the input random vector $\mathbf{X} = (X_1,X_2,\cdots,X_n)$ consisting of $n$ random variables. In other words, failure probability is the probability that the random vector $X$ lies in the unsafe region defined by g($\mathbf{X})<0$. If the joint Probability Density Function (PDF) of $\mathbf{X}$ is $f_{\mathbf{X}}( x)$, the probability of failure is evaluated using the integral
\begin{equation} \label{eq:601}
    P_f = \int_{g(x) < 0} f_{\mathbf{X}}(x) dx
\end{equation}

% In this section, the in-house built MATLAB code for probability of failure prediction using Neural-Network trained FORM/SORM method is validated with the results from literature pertaining to a straight-fiber composites case. For reference, the results from the work of Tawfik.et.al \cite{tawfik2018neural} is used for the case of a square composite laminate (a=b=1 m, a/h = 10) with deterministic ply thickness and with no cutouts. Table \ref{tab:Stat_distr_mech_prop_valid} summarizes the statistical distributions of all the input variables considered to be random (mechanical properties in GPa, material density in $kg/m^3$, ply orientation angles in degree). A stacking sequence of $[0 \degree /45\degree/-45\degree/90\degree]$ is considered for the composite plate under simply supported conditions along all 4 edges, similar to what was reported in \cite{tawfik2018neural}. A 1000 samples were generated using the statistical distribution of the input parameters given in table \ref{tab:Stat_distr_mech_prop_valid}. Out of these 1000 samples, 500 were used for training the ANN with an architecture of [11-10-1](similar to \cite{tawfik2018neural}), while the remaining 500 points were equally shared between testing and validation phase. Hyperbolic tangent activation function was used for the hidden layer (Logistic Sigmoid activation function was used for the hidden layer in Tawfik.et.al \cite{tawfik2018neural}), except for the output layer where a linear activation function is used. An $\omega_r/\omega_p = 0.97$ is used in this study. 

% %% Table : Statistical distribution of basic random variables for ANN validation with Tawfik's work
% \begin{table}[htbp!]
%     \caption{Statistical distribution of basic random variables used for validation of NN based FORM/SORM Matlab code validation \cite{tawfik2018neural}.}
%     \centering
%     \begin{tabular}{l c c c c c c c c}
%     \hline\noalign{\smallskip}
%          Property & $E_{11}$ & $E_{22}$ & $G_{12}$ & $G_{23}$ & $G_{13}$ & $\nu_{12}$ & $\rho$ & $\Delta \theta$ \\
%          \hline\noalign{\smallskip}
%          Mean & 16.48 & 1.4 & 0.87 & 0.45 & 0.87 & 0.334 & 1000 & $0 \degree$ \\
%          Std Dev & 0.61 & 0.05 & 0.052 & 0.014 & 0.052 & 0.01 & 36 & 1.8 $\degree$ \\ 
%          \hline\noalign{\smallskip}
%     \end{tabular}
%     \label{tab:Stat_distr_mech_prop_valid}
% \end{table}

% \begin{figure}[h]  
% \centering
% \includegraphics[width=0.8\textwidth]{./Figures/TVT_error_plot.eps}
% \caption{Training, Validation and Testing errors of ANN. Case for the reliability estimates w.r.t the first mode of vibration studies of a SSSS $[0\degree/45\degree/-45\degree/90\degree]$ composite plate using a [11-10-1] ANN architecture with randomness in input parameters as shown in table \ref{tab:Stat_distr_mech_prop_valid}.}
% \label{fig:TVT_error}
% \end{figure} 

\begin{table}[htbp!]
    \caption{Processing time ($T_p$) and probability of failure ($P_f$) computation using MCS and FORM-SORM-ANN methods.}
    \centering
    \begin{tabular}{c c c c c}
    \hline\noalign{\smallskip}
         COV ($\%$) & $P_f$ (MCS) & $P_f$ (ANN) & $T_p$ (MCS) & $T_p$ (ANN) \\
         \hline\noalign{\smallskip}
         1  &       &  &       &  \\
         2  & 0.035 &  & 32400 &  \\
         5  & 0.373 &  & 2900 &  \\
         8  & 0.503 &  & 1202 &  \\
         10 & 0.523 & 0.527 & 1565 &  \\
         15 & 0.547 & 0.537 & 1024 &  \\
         20 & 0.517 & 0.518 & 1172 &  \\
         \hline\noalign{\smallskip}
    \end{tabular}
    \label{tab:ANN_MCS_comparison}
\end{table}

%Once an Artificial Neural Network (ANN) had been trained with an appropriate stochastically consistent size of input-output data pairs, where the input to the Neural Network consists of random material properties, ply thickness and curved fiber angle definitions and the outputs are the random first and second mode of vibrations for free vibration case and the random critical buckling load for the buckling case, the functional representation of ANN can be further exploited to derive the first and second order derivatives of ANN outputs with any of its inputs, thereby overriding any need for symbolic calculations. 

The proposed functional approximation of the performance function and its derivatives using ANN helps to override any need for symbolic calculations.

In addition, the failure estimation was found to be the most sensitive on uncertainties in ply thickness, followed by central ply fiber orientation angle among all considered random geometric features. 

%For training the ANN, a Q4 element with 5 degrees of freedom per node, based on the FSDT is used to model the composite laminate. 

% Once this function is derived using trained ANN, its first and second order derivative of the ANN output w.r.t any of its inputs can be easily obtained, which then can be substituted into FORM and SORM formulations to predict the probability of failure of the VSCL structure along with sensitivity study. For training the ANN, a Q4 element with 5 degrees of freedom per node, based on First-order Shear Deformation Theory (FSDT) is used to model the composite laminate. 
%venkatachari2015mechanical

%Free vibration characteristics of VSCL plates/shells have been numerically studied using a higher order accurate theory by Anand.et.al \cite{venkatachari2018variable}. This study was further extended to take into account the environmental effects and inclusion of cutouts in \cite{venkatachari2016environmental}. A systematic assessment of higher-order structural models for bending analysis of VSCL was carried out in \cite{venkatachari2014assessment}. 

% The effect of temperature distributions on the buckling behavior of VSCL plates using first order shear deformation theory was studied in \cite{manickam2018thermal,venkatachari2015mechanical}. 

% The natural modes of VSCL plates with curvilinear fibers using the $p$-version finite element, that follows a third order deformation theory, was examined in \cite{akhavan2011natural}. Aeroelastic studies of VSCL plates, which falls under the classification of eigenvalue problems, was studied in the presence of supersonic flow in \cite{akhavan2018aeroelasticity}. Geometric non-linear vibration studies of VSCL plates, wherein the vibration amplitudes are not small when compared to the plate thickness, was studied using First-order Shear Deformation Theory (FSDT) in \cite{ribeiro2012non}. Dynamics instability of VSCL plates using Rayleigh-Ritz method was considered in \cite{loja2017dynamic}.


%Numerical investigation into stochastic vibration behaviour of long fibre reinforced composites under uncertainty in fibre orientations was done in \cite{sepahvand2016spectral}. A similar spectral stochastic finite element approach for static analysis of fiber reinforced composite plates under material uncertainties represented using random field theory was investigated in \cite{chen2008spectral}. Given the scope of the present work being limited to reliability studies of composite structures under multiple uncertainties, a comprehensive review on the same was first presented in \cite{chiachio2012reliability}. 

% Reliability analysis, being an extension of the forward uncertainty propagation modelling in the presence of a performance function, of composite laminates under static loads or free vibrations can be performed using different techniques. 

% A mean-centered second-moment method to study the free vibration and reliability study of composite cantilevers was done in \cite{oh1997free}. A stochastic finite element method for the analysis of composite plates was proposed in \cite{haldar2000probability}. A First Order Reliability Method (FORM) to study shear deformable laminated composite plates was used in \cite{gosling2014high}. 

% Typically, a neural network gets trained with a few samples from a high-dimensional parametric space obtained by the conventional Monte Carlo techniques, and then the trained ANN is used to make predictions. 

Section \ref{Sec3} introduces the reader to importance sampling based reliability estimation, against which our proposed method results are validated. A basic introduction to an ANN architecture is provided in section \ref{Sec4} along with the details on how to derive the first and second order derivatives of the ANN derived mapping function between its input-output pairs. With this knowledge, section \ref{Sec6} introduces the concept of FORM and SORM and how the ANN function derivatives can be substituted in these reliability formulations to approximate the failure probability predictions. An additional post-processing step using the weights of the trained ANN for sensitivity analysis is also elucidated in this section. Numerical examples are provided in section \ref{Sec8} to demonstrate the accuracy of the proposed implementation,

%Although there is no hard and fast rule on its choice, it has been found that a standard normal PDF centered on the Maximum Probability of failure Point (MPP) obtained using FORM in the space of independent standardized random variables can be a good candidate for the proposal distribution \cite{melchers1989importance}. Moreover, IS is not sensitive to the exact position of MPP. 

The procedure to carry out a sensitivity analysis using the trained ANN so as to determine the relative importance of the various model inputs is described next. This is based on the method proposed in \cite{Garson:1991:INC:129449.129452}. This method involves partitioning the hidden-output connection weights of each hidden node into components associated with each input node \cite{Chok}.

The sensitivity computation process as proposed by \cite{Garson:1991:INC:129449.129452} is as follows: 

\begin{itemize}
    \item As a first step, products $P_{ij}$ are obtained by multiplying the absolute value of the connection weight between the hidden node i and output layer neuron, with the absolute value of the connection weight between the hidden node i to the j'th input variable. For example, $P_{11}$ corresponds to the product of connection weights between neuron 1 in hidden layer to the output layer neuron and neuron 1 in the hidden layer to the 1st input variable.  
    
    \item For the i'th hidden layer neuron, divide $P_{ij}$ by the sum of all the input variables to obtain $Q_{ij}$. For example, 
    \begin{equation}
        Q_{11} = \frac{P_{11}}{\sum_{j=1}^{N}P_{1j}}
    \end{equation}
    \noindent where $N$ is the number of input variables. 
    
    \item Next, for each input variable node $j (j=1,\cdots,N)$, we then calculate $S_j$ as follows: 
    
    \begin{equation}
        S_{j} = \sum_{k=1}^{N_h} Q_{kj}
    \end{equation}
    \noindent where $N_h$ is the number of neurons in hidden layer. 
    
    \item Finally, the relative importance (or the sensitivity index) of the j'th input variable is calculated by dividing $S_j$ with the sum of all the input variable contributions as shown below. 
    
    \begin{equation} \label{eq:TotalEffectIndic}
        SI_{j} = \frac{S_j}{\sum_{j=1}^N S_j}
    \end{equation}
\end{itemize}
